MajorityNets: BNNs Utilising Approximate Popcount for Improved Efficiency

Binarized neural networks (BNNs) have shown exciting potential for utilising neural networks in embedded implementations where area, energy and latency constraints are paramount. With BNNs, multiply-accumulate (MAC) operations can be simplified to XnorPopcount operations, leading to massive reductions in both memory and computation resources. Furthermore, multiple efficient implementations of BNNs have been reported on field-programmable gate array (FPGA) implementations. This paper proposes a smaller, faster, more energy-efficient approximate replacement for the XnorPopcountoperation, called XNorMaj, inspired by state-of-the-art FPGAlook-up table schemes which benefit FPGA implementations. Weshow that XNorMaj is up to 2x more resource-efficient than the XnorPopcount operation. While the XNorMaj operation has a minor detrimental impact on accuracy, the resource savings enable us to use larger networks to recover the loss.

==> BackUp_Background_Quantization.tex <==
\subsection{Quantization and Binarized Neural Networks}
In this section we briefly review quantization techniques and their application to BNN accelerators. A more comprehensive survey is available in~\cite{DBLP:journals/csur/WangDZNNLCC19}.

Quantization has been extensively studied in the context of DNN implementations since it offers a massive reduction in both memory footprint and computation requirements leading to smaller, faster, and more energy-efficient implementations, especially for mobile applications, which is the concern of this paper. In this process, data is mapped to a lower-precision format with a smaller set of quantization levels. Recently, Guo~et~al.~\cite{DBLP:journals/trets/GuoZYWY18} demonstrated that using 8 bits or more for inference task produces insignificant accuracy drop, while 6 bits causes noticeable accuracy degradation. 

Low-precision computation can be beneficial on all platforms. CPUs and GPUs generally support up to 8-bit integer operations while the recent Nvidia Turing architecture supports INT4 natively~\cite{Nvidia:Turing}. Several recent ASIC accelerators have employed low-precision arithmetic, {\em e.g.} Google's TPU~\cite{DBLP:conf/isca/JouppiYPPABBBBB17} and Bit-brick~\cite{DBLP:conf/isca/SharmaPSLCCE18}. Since FPGAs employ fine-grained datapaths, low precision is advantageous. An analyze on FPGA resource usage for different bit-width computations can be found in~\cite{DBLP:journals/corr/abs-1712-08934}. 

Most FPGA accelerators use fixed-point computations, {\em e.g.} 16~bit fixed-point computation has been widely adopted \cite{DBLP:conf/fpga/QiuWYGLZYTXSWY16,DBLP:conf/fccm/GuanLXWSCSZC17,DBLP:conf/iccad/ZhangFZPC16}, 12~bit weights were used in ESE~\cite{DBLP:conf/fpga/HanKMHLLXLYWYD17}, and 8~bit units employed in~\cite{DBLP:journals/tcad/GuoSQYWYHWY18}. The evolution of FPGA-accelerators for inference has been moving towards extremely low-precisions where FPGAs can outperform GPUs in terms of throughput and latency. Li~et~al.~\cite{DBLP:journals/corr/LiL16} proposed ternarized neural networks (TNNs), in which the weights are restricted to plus/minus a scale value and zero. In this case, the multiplication in a MAC operation can be avoided~\cite{DBLP:conf/fpl/Prost-BoucleBPA17}. 
Binarization, the highest degree of quantization, represents model parameters and input activations by a single bit, with logic 1 and 0 representing the values 1 and -1 respectively. Courbariaux~et~al.~\cite{DBLP:journals/corr/CourbariauxBD15}, in BinaryConnect (BC), proposed binarization of weights and keeping a higher activation precision, which reduces the majority of MAC operations to addition and subtraction. As a followup, Courbariaux~et~al.~\cite{DBLP:journals/corr/CourbariauxB16} applied binarization to both weights and activations. In this case, multiplication is replaced by the Xnor operation, and summation replaced by counting the number of 1 values (popcount). In this case, MACs are replaced with the much simpler XnorPopcount operation. Although the accuracy drop of BC and BNN on the ImageNet dataset were 19\% and 29.8\% respectively, these ideas enabled significant improvements in resource, latency, and power. 

To deal with the accuracy drop of BNNs, Rastegari~et~al.~\cite{DBLP:conf/eccv/RastegariORF16} proposed XNOR-Net, in which extra scaling layers were placed after the binarized convolution layers to recover the dynamic range. XNOR-Net enhanced speed and memory footprint by  58$\times$ and 32$\times$ respectively, with the 12.4\% accuracy drop compared to the fully floating point implementation of AlexNet on the ImageNet dataset. Recently, RebNet~\cite{DBLP:journals/corr/abs-1711-01243} used a multi-bit activation structure based on XnorPopcount, which can effectively recover the accuracy. Similar approaches using 2~bit activation can be found in  DoReFa-Net~\cite{DBLP:journals/corr/ZhouNZWWZ16} and HWGQ-Net~\cite{DBLP:conf/cvpr/CaiHSV17}.

%CPUs and GPUs are not efficient platforms for BNNs. However, a GPU efficient implementation of BNNs is reported in~\cite{DBLP:conf/eusipco/KhanHB18}. 
FPGA and ASIC are the promising platforms for the implementation of binarized networks%binarized weight networks (BWNs) and BNNs
~\cite{DBLP:conf/fpga/NurvitadhiVSMHH17}. Moreover, FPGAs offer improved efficiency over CPUs and GPUs while being more customizable than ASICs~\cite{DBLP:conf/fpl/MossNSMMSL17}. %,DBLP:conf/fpt/NurvitadhiSSMVM16}. 
Xnor-Bin~\cite{DBLP:journals/corr/abs-1803-05849} is the state of the art ASIC implementation on 65nm, which can maintain all parameters of an AlexNet sized network on-chip and achieve 95~TOPs. % and compare to state of the art FPGA implementation, FINN~\cite{DBLP:conf/fpga/UmurogluFGBLJV17}, it is 168X more power efficient.
YodaNN~\cite{DBLP:journals/corr/AndriCRB16} and BRein~\cite{8226999} are two other high-performance ASIC implementations. % using BWN and BNN architectures. Moss~et~al.~\cite{DBLP:conf/fpl/MossNSMMSL17} implemented a high-performance CPU-FPGA BNN system. 
Liang~et~al.~\cite{DBLP:journals/ijon/LiangYLLW18} proposed FP-BNN, based on Xnor-shift multipliers, which is the state-of-the-art FPGA-based BNN implementation. Also, an efficient embedded implementation using XnorPopcount and thresholding can be find in~\cite{DBLP:conf/fpga/UmurogluFGBLJV17}. Recently using the binarized version of efficient convolution kernels such as depth-wise separable convolution~\cite{DBLP:conf/isvlsi/HeARF18} is getting interests which offer new trade-offs. However, in these approaches, accuracy degradation is noticeable yet. Other implementations can be found in~\cite{DBLP:conf/fpt/NurvitadhiSSMVM16,DBLP:conf/fpga/LiLXYR17,DBLP:conf/fpl/NakaharaFS17,DBLP:conf/fpga/ZhaoSZXLSGZ17,DBLP:conf/islped/YangHF18}

